PO-EMO: Conceptualization, Annotation, and Modeling of Aesthetic Emotions in German and English Poetry

Most approaches to emotion analysis of social media, literature, news, and other domains focus exclusively on basic emotion categories as defined by Ekman or Plutchik. However, art (such as literature) enables engagement in a broader range of more complex and subtle emotions. These have been shown to also include mixed emotional responses. We consider emotions in poetry as they are elicited in the reader, rather than what is expressed in the text or intended by the author. Thus, we conceptualize a set of aesthetic emotions that are predictive of aesthetic appreciation in the reader, and allow the annotation of multiple labels per line to capture mixed emotions within their context. We evaluate this novel setting in an annotation experiment both with carefully trained experts and via crowdsourcing. Our annotation with experts leads to an acceptable agreement of kappa = .70, resulting in a consistent dataset for future large scale analysis. Finally, we conduct first emotion classification experiments based on BERT, showing that identifying aesthetic emotions is challenging in our data, with up to .52 F1-micro on the German subset. Data and resources are available at https://github.com/tnhaider/poetry-emotion

==> tables/authors_corpora.tex <==
\begin{table}[]
\begin{scriptsize}
\begin{tabular}{ll||ll}
English & Birth & German & Frequency \\
\hline
AlexanderPope   & 1688            &  &    \\
AlfredLordTennyson & 1809       &  &    \\
AnneKilligrew & 1660           &  &    \\
EdmundSpenser & 1552            &  &    \\
EdwardEstlinCummings & 1894     &  &    \\
ElizabethBarrettBrowning & 1806 &  &    \\
EmilyDickinson & 1830           &  &    \\
JohnDonne & 1572               &  &    \\
JohnDryden & 1631               &  &    \\
JohnKeats & 1795                &  &    \\
JohnMilton & 1608               &  &    \\
PercyByssheShelley & 1792       &  &    \\
RobertBurns & 1759           &  &    \\
RobertFrost & 1874              &  &    \\
RudyardKipling & 1865           &  &    \\
Shakespeare & 1564              &  &    \\
ThomasStearnsEliot & 1888       &  &    \\
WaltWhitman & 1819              &  &    \\
WilliamBlake & 1757             &  &    \\
WilliamButlerYeats & 1865       &  &    \\
WilliamCarlosWilliams & 1883    &  &    \\
WilliamWordsworth & 1770        &  &    \\
\end{tabular}
\end{scriptsize}
\end{table}

==> tables/emotionlabels.tex <==
\begin{table*}[!htb]
\begin{small}
    \centering
    \begin{tabular}{l|l|l}
    Final set & Initial Set & Items \\
    \hline
    Beauty/Joy  & Beauty        & (beautiful / pleasing)\\ 
                & Joy           & (makes happy / joyful)\\
    Annoyance   & Anger         & (annoys / angers me/ frustrated) \\
    Awe/Sublime & Awe/Sublime   & (overwhelming / sense of greatness) \\
    Humor       & Humor         & (funny / amusing) \\
    Sadness     & Sadness       & (makes sad / touches me) \\
    Suspense    & Suspense / Anticipation & (found it gripping / sparked interest) \\
    Vitality / Stimulation / Activation   & Vitality      & (found invigorating / spurs on / inspires) \\
    Nostalgia-Sad/Nostalgia-Joy & Nostalgia & (makes nostalgic) \\
    Uneasiness  & Uneasiness    & (found unsettling / disturbing / frightening) \\
                & Ugliness      & (found ugly / distasteful) \\
                & Disgust       & ? \\
        &  Confusion    & (confuses / hard to understand)  \\
        &  Boredom      & (bores me) \\
        &  Other        & \\
    \end{tabular}
    \caption{Emotion Labels with Items}
    \label{tab:labels}
    \end{small}
\end{table*}

==> tables/pics/crowdsVsExperts.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4250.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(688,871){\makebox(0,0)[r]{\strut{}$0.12$}}%
      \csname LTb\endcsname%
      \put(688,1231){\makebox(0,0)[r]{\strut{}$0.14$}}%
      \csname LTb\endcsname%
      \put(688,1590){\makebox(0,0)[r]{\strut{}$0.16$}}%
      \csname LTb\endcsname%
      \put(688,1949){\makebox(0,0)[r]{\strut{}$0.18$}}%
      \csname LTb\endcsname%
      \put(688,2309){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%
      \put(688,2668){\makebox(0,0)[r]{\strut{}$0.22$}}%
      \csname LTb\endcsname%
      \put(688,3027){\makebox(0,0)[r]{\strut{}$0.24$}}%
      \csname LTb\endcsname%
      \put(1181,352){\makebox(0,0){\strut{}4}}%
      \csname LTb\endcsname%
      \put(1975,352){\makebox(0,0){\strut{}6}}%
      \csname LTb\endcsname%
      \put(2770,352){\makebox(0,0){\strut{}8}}%
      \csname LTb\endcsname%
      \put(3564,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1859){\rotatebox{-270}{\makebox(0,0){\strut{}Average $\kappa$}}}%
      \put(2372,112){\makebox(0,0){\strut{}Crowd Workers $N$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{tables/pics/crowdsVsExperts.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> tables/pics/dist_de.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4250.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(496,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(496,779){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(496,1047){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(496,1314){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(496,1582){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(496,1849){\makebox(0,0)[r]{\strut{}$50$}}%
      \csname LTb\endcsname%
      \put(496,2117){\makebox(0,0)[r]{\strut{}$60$}}%
      \csname LTb\endcsname%
      \put(496,2384){\makebox(0,0)[r]{\strut{}$70$}}%
      \csname LTb\endcsname%
      \put(496,2652){\makebox(0,0)[r]{\strut{}$80$}}%
      \csname LTb\endcsname%
      \put(496,2919){\makebox(0,0)[r]{\strut{}$90$}}%
      \csname LTb\endcsname%
      \put(812,352){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%
      \put(1398,352){\makebox(0,0){\strut{}2}}%
      \csname LTb\endcsname%
      \put(1984,352){\makebox(0,0){\strut{}3}}%
      \csname LTb\endcsname%
      \put(2569,352){\makebox(0,0){\strut{}4}}%
      \csname LTb\endcsname%
      \put(3155,352){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%
      \put(3741,352){\makebox(0,0){\strut{}6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1715){\rotatebox{-270}{\makebox(0,0){\strut{}in \%}}}%
      \put(2276,112){\makebox(0,0){\strut{}Number of Emotions}}%
      \put(2276,3159){\makebox(0,0){\strut{}German}}%
      \put(3226,2776){\makebox(0,0)[r]{\strut{}line}}%
      \csname LTb\endcsname%
      \put(3226,2616){\makebox(0,0)[r]{\strut{}stanza}}%
      \csname LTb\endcsname%
      \put(3226,2456){\makebox(0,0)[r]{\strut{}poem}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{tables/pics/dist_de.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> tables/pics/dist_en.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4250.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(496,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(496,856){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(496,1200){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(496,1544){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(496,1887){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(496,2231){\makebox(0,0)[r]{\strut{}$50$}}%
      \csname LTb\endcsname%
      \put(496,2575){\makebox(0,0)[r]{\strut{}$60$}}%
      \csname LTb\endcsname%
      \put(496,2919){\makebox(0,0)[r]{\strut{}$70$}}%
      \csname LTb\endcsname%
      \put(812,352){\makebox(0,0){\strut{}1}}%
      \csname LTb\endcsname%
      \put(1398,352){\makebox(0,0){\strut{}2}}%
      \csname LTb\endcsname%
      \put(1984,352){\makebox(0,0){\strut{}3}}%
      \csname LTb\endcsname%
      \put(2569,352){\makebox(0,0){\strut{}4}}%
      \csname LTb\endcsname%
      \put(3155,352){\makebox(0,0){\strut{}5}}%
      \csname LTb\endcsname%
      \put(3741,352){\makebox(0,0){\strut{}6}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1715){\rotatebox{-270}{\makebox(0,0){\strut{}in \%}}}%
      \put(2276,112){\makebox(0,0){\strut{}Number of Emotions}}%
      \put(2276,3159){\makebox(0,0){\strut{}English}}%
      \put(3226,2776){\makebox(0,0)[r]{\strut{}line}}%
      \csname LTb\endcsname%
      \put(3226,2616){\makebox(0,0)[r]{\strut{}stanza}}%
      \csname LTb\endcsname%
      \put(3226,2456){\makebox(0,0)[r]{\strut{}poem}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{tables/pics/dist_en.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup

